Efficient Availability Attacks against Supervised and Contrastive Learning Simultaneously

Availability attacks can prevent the unauthorized use of private data and commercial datasets by generating imperceptible noise and making unlearnable examples before release. Ideally, the obtained unlearnability prevents algorithms from training usable models. When supervised learning (SL) algorithms have failed, a malicious data collector possibly resorts to contrastive learning (CL) algorithms to bypass the protection. Through evaluation, we have found that most of the existing methods are unable to achieve both supervised and contrastive unlearnability, which poses risks to data protection. Different from recent methods based on contrastive error minimization, we employ contrastive-like data augmentations in supervised error minimization or maximization frameworks to obtain attacks effective for both SL and CL. Our proposed AUE and AAP attacks achieve state-of-the-art worst-case unlearnability across SL and CL algorithms with less computation consumption, showcasing prospects in real-world applications.

==> files/impact.tex <==
\section*{Impact Statement}
% This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.

This paper presents work whose goal is to advance the field of availability attacks. %Machine Learning.
Although availability attacks we investigate are a form of data poisoning attack, due to their nature of indiscriminate attack, they are often considered in the literature as a data protection method that helps data owners prevent the misuse of privacy data or business data. Furthermore, our research can enable us to better understand the vulnerabilities of different machine learning algorithms, thereby promoting further research in the field of AI security and safety.

